Distributed Automatic Load-Frequency Control with Optimality in Power Systems

With the increasing penetration of renewable energy resources, power systems face new challenges in balancing power supply and demand and maintaining the nominal frequency. This paper studies load control to handle these challenges. In particular, a fully distributed automatic load control (ALC) algorithm, which only needs local measurement and local communication, is proposed. We prove that the load control algorithm globally converges to an optimal operating point which minimizes the total disutility of users, restores the nominal frequency and the scheduled tie-line power flows, and respects the load capacity limits and the thermal constraints of transmission lines. It is further shown that the asymptotic convergence still holds even when inaccurate system parameters are used in the control algorithm. In addition, the global exponential convergence of the reduced ALC algorithm without considering the capacity limits is proved and leveraged to study the dynamical tracking performance and robustness of the algorithm. Lastly, the effectiveness, optimality, and robustness of the proposed algorithm are demonstrated via numerical simulations.

==> Convergence.tex <==
\section{Asymptotic Convergence Analysis} \label{sec:convergence}

%In this section, the proofs of Theorems \ref{thm1} and \ref{thm2} are provided as the convergence analysis for the ALC algorithm.














==> Convergence_uncertainD.tex <==
\section{Convergence under Uncertain Parameters $D_i$}

A particular challenge associated with implementing \eqref{cm:r_derivative} of the proposed control law is that the damping coefficient $D_i$ is in general hard to be known exactly. In this section, it is shown that the system under the proposed control law still converges to the same optimal equilibrium as that in Section \ref{sec:convergence}, given that the uncertainty in $D_i$ is small enough.  

To this end, assume that an inaccurate damping coefficient $D'_i = D_i + \delta a_i$, where $\delta a_i$ is the uncertainty, is used instead of $D_i$ in \eqref{cm:r_derivative}. The proposed control law \eqref{cm} and the network dynamics \eqref{dynamic} are then equivalent to the primal and dual gradient algorithm \eqref{sol}--\eqref{gra} except that \eqref{gra:virtual_freq} is now:
\begin{eqnarray}
\dot{\mu}_i&=& \epsilon_{\mu_i}\left(-d_i+P^{in}_i + \delta a_i \omega_i -\sum_{j:ij\in\mathcal{E}_{in}}B_{ij}\left(\psi_{i}-\psi_j\right) \right.
\nonumber \\
&& \left. \ \ \qquad\qquad\qquad +\sum_{k:ki\in \mathcal{E}_{in}}B_{ki}\left(\psi_k-\psi_i\right)\right) \label{eq:virtual_freq_uncertainD}
\end{eqnarray} 
with the additional term $\delta a_i \omega_i$. 

We prove stability of the system under uncertainty in $D_i$ with the following modifications to the proposed control law:

\noindent i) The cost function $C_i(d_i) \rightarrow +\infty$ as $d_i\rightarrow \overline d_i^{-}$ or $ \underline d_i^{+} \leftarrow d_i$; see \cite{the}. As a result, $\gamma_i^+(t) \equiv \gamma_i^-(t) \equiv 0$ for all $t \geq 0$ if the initial values of $\gamma_i^+$ and $\gamma_i^-$ are zero for all $i \in \mathcal{N}$. Therefore the dynamics of $\gamma^+$ and $\gamma^-$ can be ignored.    

\noindent ii) The control law \eqref{gra:d} is modified to the following:
\begin{eqnarray}
d_i &=& \left(C_i^{'}\right)^{-1} \left(\lambda_i+\mu_i \right), \quad \forall i \in \mathcal{N}. \label{eq:d_control_instant}
\end{eqnarray}

It will be explained later why we need the modifications above to prove stability of the closed-loop system under uncertainty in $D_i$. Corresponding to these modifications, define $(d,\zeta):=\left(d, x,\lambda_{\mathcal{G}},\mu,\sigma \right)=(d, P, \psi, \lambda_{\mathcal{G}},\mu, \sigma)$ and the following function of $\zeta$:
\begin{eqnarray}
\tilde L(\zeta) := \min_{d} \overline L(d, \zeta) \nonumber
\end{eqnarray}
where the minimizer $d$ is given by \eqref{eq:d_control_instant} and satisfies:
\begin{eqnarray}
\frac{\partial\bar{L}}{\partial d}(d,\zeta) = 0. \nonumber
\end{eqnarray}

The modified closed-loop system under uncertain $D_i$, described by \eqref{sol}, \eqref{gra:lambda}, \eqref{gra:P}, \eqref{gra:psi}, \eqref{gra:sigma_plus}, \eqref{gra:sigma_minus}, \eqref{eq:virtual_freq_uncertainD}, \eqref{eq:d_control_instant}, can be written as:   
\begin{align} \label{dyn_uncertianD}
\begin{split}
&\dot{x}=-\Xi_x\frac{\partial\tilde{L}}{\partial x}, \quad
\dot{\lambda}_\mathcal{G}=\Xi_{\lambda_\mathcal{G}}\frac{\partial\tilde{L}}{\partial \lambda_\mathcal{G}}\\ 
&\dot{\mu}=\Xi_\mu\left[\frac{\partial\tilde{L}}{\partial \mu} + \delta A \lambda \right], \quad \ \,
\dot{\sigma}=\Xi_{\sigma}\left[\frac{\partial\tilde{L}}{\partial {\sigma}}\right]^+_{\sigma}
\end{split}
\end{align}
where $\delta A:=\mathrm{diag}(\delta a_i, ~i\in \mathcal{N})$. The system \eqref{dyn_uncertianD} can be written more compactly as:
\begin{eqnarray} \label{dyn_uncertianD_compact}
\dot \zeta &=& \Xi_\zeta \left[ f(\zeta) \right]_\sigma^+
\end{eqnarray}
where $\Xi_\zeta:=\mathrm{blockdiag}(\Xi_x, \Xi_{\lambda_\mathcal{G}}, \Xi_\mu, \Xi_\sigma)$, and 
\begin{eqnarray}\nonumber
f(\zeta):=\left[ -\frac{\partial\tilde{L}}{\partial x}^T,  \frac{\partial\tilde{L}}{\partial \lambda_\mathcal{G}}^T, \left(\frac{\partial\tilde{L}}{\partial \mu} + \delta A \lambda \right)^T,  \frac{\partial\tilde{L}}{\partial {\sigma}}^T\right]^T.
\end{eqnarray}
Note that in the vector $\lambda=(\lambda_\mathcal{L}, \lambda_\mathcal{G})$, only $\lambda_\mathcal{G}$ is a variable of the system \eqref{dyn_uncertianD} or \eqref{dyn_uncertianD_compact}, whereas $\lambda_\mathcal{L}$ is the abbreviation of a vector-valued function $\lambda_\mathcal{L}(\zeta)$ defined by the equation:\footnote{The $|\mathcal{N}|$-by-$|\mathcal{E}|$ matrix $C$ is the incidence matrix of the power network, and $C_{\mathcal{L}}$ is the submatrix of $C$ composed only of the rows corresponding to the load buses in $\mathcal{L}$.}
\begin{eqnarray}\label{eq:lambda_L_def}
 P^{in}_\mathcal{L} -D_{\mathcal{L}} \lambda_\mathcal{L}  - d_{\mathcal{L}}\left(\lambda_\mathcal{L} + \mu_\mathcal{L}  \right) -C_{\mathcal{L}} P = 0
\end{eqnarray}
where $d_{\mathcal{L}}\left(\lambda_\mathcal{L} + \mu_\mathcal{L} \right)$ is defined by \eqref{eq:d_control_instant}. 

The stability result for the system under uncertain $D_i$ is formally given as the following theorem.

\begin{theorem}\label{thm:stability_uncertain_D}
Assume that the cost function $C_i(d_i)$ is $\alpha$-strongly convex and second-order continuously differentiable ($C_i \in C^2$ with $C''_i(d_i) \geq \alpha >0$) in the interior of its domain $(\underline d_i, \overline d_i)$, and $C_i(d_i) \rightarrow +\infty$ as $d_i\rightarrow \overline d_i^{-}$ or $ \underline d_i^{+} \leftarrow d_i$. Moreover, assume that the functions $C'_i$ are Lipschitz continuous with Lipschitz constant $L>0$. Then the system \eqref{dyn_uncertianD_compact} converges to an optimum of problem \eqref{op} whenever 
\begin{eqnarray}\label{eq:cond_uncertainty_D}
\delta a_i \in 2\left( \underline d' - \sqrt{\underline d'^2 + \underline d' D_{\mathrm{min}}}, \underline d' + \sqrt{\underline d'^2 + \underline d' D_{\mathrm{min}}}\right)
\end{eqnarray}
where $\underline d' := 1/L$ and $D_{\mathrm{min}}:=\min_{i \in \mathcal{N} } D_i$. 
\end{theorem}

The condition and result of Theorem \ref{thm:stability_uncertain_D} are the same as those of \cite[Theorem 15]{the}, and their proofs follow the same techniques. Therefore, we only provide a sketch of proof for Theorem \ref{thm:stability_uncertain_D}. 

Consider a Lyapunov function candidate
\begin{eqnarray}\nonumber
U(\zeta) = \frac{1}{2} \left(\zeta - \zeta^*\right)^T  \Xi_{\zeta}^{-1} \left(\zeta- \zeta^*\right).
\end{eqnarray}
We first show that under the dynamics \eqref{dyn_uncertianD_compact}, the time derivative of $U(\zeta)$ is upper-bounded by:
\begin{eqnarray}\nonumber
\dot U(\zeta) \leq \int_0^1 (\zeta-\zeta^*)^T [H(\zeta(s))](\zeta-\zeta^*) ds
\end{eqnarray} 
where $\zeta(s) = \zeta^* +s (\zeta- \zeta^*)$, and $H(\zeta)$ is given by a block matrix which is zero everywhere except:

\noindent i) a block corresponding to variables $(P, \mu_\mathcal{L})$, which is the same as $H_{P,\lambda_\mathcal{L}}(z)$ in \cite{the}; 

\noindent ii) a block corresponding to variables $(\mu_\mathcal{G}, \lambda_\mathcal{G})$, which is the same as $H_{\lambda_\mathcal{G}, \nu_\mathcal{G}}(z)$ in \cite{the}.

Therefore, under the condition \eqref{eq:cond_uncertainty_D}, the matrix $H(\zeta)$ is negative semi-definite. Applying the invariance principle, the convergence result in Theorem \ref{thm:stability_uncertain_D} can be proved. 

\textbf{Discussion.} \emph{Why $\gamma^+$ and $\gamma^-$ are ignored for stability proof under uncertain $D_i$?} 
If we consider \eqref{gra:gamma_plus} and \eqref{gra:gamma_minus}, then instead of proving negative semi-definiteness of the block matrices corresponding to $(P, \mu_\mathcal{L})$ and $(\mu_\mathcal{G}, \lambda_\mathcal{G})$, we have to prove negative semi-definiteness of the block matrices corresponding to $(P, \mu_\mathcal{L}, \gamma^+_\mathcal{L}, \gamma^-_\mathcal{L})$ and $(\mu_\mathcal{G}, \lambda_\mathcal{G}, \gamma^+_\mathcal{G}, \gamma^-_\mathcal{G})$. However, one can show that these two larger block matrices have strictly positive eigenvalues for arbitrarily small $\delta A$, which makes the proof technique fail.

\emph{Why the control law is modified from the derivative form \eqref{gra:d} to the stationary form \eqref{eq:d_control_instant}?}
With the derivative form \eqref{gra:d}, one can show that in $H(\zeta)$, the block at the diagonal position corresponding to $\mu$ is zero, and hence it is impossible to make $H(\zeta)$ negative semi-definite when the off-diagonal blocks containing $\delta A$ are non-zero.
}
